Crowd Coach: Peer Coaching for Crowd Workers' Skill Growth

Traditional employment usually provides mechanisms for workers to improve their skills to access better opportunities. However, crowd work platforms like Amazon Mechanical Turk (AMT) generally do not support skill development (i.e., becoming faster and better at work). While researchers have started to tackle this problem, most solutions are dependent on experts or requesters willing to help. However, requesters generally lack the necessary knowledge, and experts are rare and expensive. To further facilitate crowd workers' skill growth, we present Crowd Coach, a system that enables workers to receive peer coaching while on the job. We conduct a field experiment and real world deployment to study Crowd Coach in the wild. Hundreds of workers used Crowd Coach in a variety of tasks, including writing, doing surveys, and labeling images. We find that Crowd Coach enhances workers' speed without sacrificing their work quality, especially in audio transcription tasks. We posit that peer coaching systems hold potential for better supporting crowd workers' skill development while on the job. We finish with design implications from our research.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

==> cscwOld.tex <==
\section{Introduction}
In traditional employment, individuals usually have the opportunity to grow their skills and careers over time \cite{pew2013civic,williamson1998lifeworlds,duyff1999value, billett2001learning}. Work satisfaction theories have stressed the importance of fostering personal and professional growth in work environments to increase workers' motivations and satisfaction \cite{billett2001learning, ramlall2004review, ryan2000self, cartwright2006meaning}. This desire to grow professionally is also present in crowd workers \cite{kaufmann2011more}. However, crowd markets in general have not been designed for professional development \cite{bigham2017scopist,dontcheva2014combining,whiting2016crowd,Micro-internships, suzuki2016atelier}. Consequently, crowd workers who wish to extend their skills must explore ways to train themselves outside crowdsourcing platforms \cite{kittur2013future}. But, given the notoriously low pay of crowd work \cite{paolacci2010running, berg2015income, durward2016crowd, thies2011paid, hara2017data}, requiring workers to use additional time and financial resources for professional development is impractical \cite{kelliher2008better,van2017platform,rosenblat2016algorithmic,alkhatib2017examining}.

To address this problem, scholars have very recently started to explore models to enable professional growth while doing crowd work \cite{dontcheva2014combining, coetzee2015structuring, doroudi2016toward}. Research has showed that these models can help crowd workers to improve. But, these models have also relied heavily on domain experts and even requesters, whose time is limited and are expensive to hire \cite{suzuki2016atelier}. Requesters also generally have insufficient knowledge or motivation for helping crowd workers \cite{doroudi2016toward,irani2013turkopticon,kulkarni2012turkomatic}. Consequently, requester or expert driven assistance is scarce and does not always address  workers' needs \cite{}. 

Our goal in this work is to understand the process by which crowd workers currently improve their skills on crowd markets without the aid of experts or requesters, and to support this process by introducing a novel tool that facilitates crowd workers' professional development. 

To understand the process, we build on early survey research \cite{} on how crowd workers develop skills on Amazon Mechanical Turk (AMT). 
We find that crowd workers usually want to develop their audio transcription skills (especially because these tasks have the highest pay rate). To figure out how to become better at AMT tasks, crowd workers usually rely on short forum posts from their peers. However, finding such advice can be time-consuming and workers usually have a hard time remembering to apply to their crowd work the advice they read on the forum. 

Armed with the knowledge that workers found short quick advice from peers helpful for self-improvement on AMT, we designed a tool to support workers' professional growth while on the job. The tool, \sys is a chrome plugin that provides workers with short micro-advice from peers while completing a task on AMT. \sys provides two primary mechanisms to support skill development on crowd markers: Micro-Coaching and Selective Advice. \sys's interface encourages workers to provide short snippets of advice to each other (no more than 100 characters). This approach draws on ``Twitch crowdsourcing'' research \cite{} where in seconds people can rapidly complete a micro-task. \sys's design enables workers to micro-coach others without having to invest much time. In parallel \sys's Selective Advice enables workers to focus on the advice that will help them the most to grow professionally. 

In this paper we contribute: 1) an investigation of crowd workers' practices for developing their skills on AMT; 2) a system supporting workers' skill development; 3) a mechanism that enables rapidly providing and receiving coaching while doing crowd work; and 4) a field experiment and studies demonstrating that \sys enables peer-coaching and benefits workers receiving the coaching. 
We believe \sys's method of using short, selective peer coaching has great potential for transforming the ways in which crowd workers can grow and develop in their labor. 

\section{Related Work}

\sys's system design is informed by two main research areas: (1) skill development in crowd work, (2) tools for improving crowdsourcing platforms.


\subsection{Skill Development in Crowd Work}

Both researchers and practitioners still struggle with enabling skill development on crowdsourcing platforms 
\cite{deng2013crowdsourcing, thies2011paid}. Enabling skill develop is important for several reasons: first skill improvement enhances performance in crowd work \cite{kittur2013future}. Complex tasks also need skilled workers to complete them \cite{noronha2011platemate}. Having more specialized workers can facilitate the completion of more work and facilitate reaching  more complex goals \cite{}. Second, skill development can help crowd workers to finish their tasks faster \cite{}. This can potentially aid crowd workers to obtain a higher hourly pay, as payment on AMT is typically based on workload (number of tasks completed)\cite{}. Third, ``learning new skills'' is one of the main motivators that crowd workers have for joining the crowd market \cite{kaufmann2011more}. Crowd workers expect that their experiences on crowdsourcing platforms will benefit their career development \cite{brabham2008crowdsourcing}. Nevertheless, most crowd workers lack the opportunity for improving or advancing their careers \cite{suzuki2016atelier}.     

To address this problem researchers have developed tools to facilitate skill development in crowd work. Atelier for Upwork \cite{suzuki2016atelier} provided a mentorship model where experts helped crowd workers learn new skills; LevelUp for Photoshop \cite{dontcheva2014combining} integrated tutorials designed by experts to teach people designer skills while completing basic photograph improvement tasks. However, most of these tools require that experts invest their time in helping new workers, either via mentoring or by developing educational material such as tutorials. Yet, experts' time is limited and expensive \cite{}. 

To reduce the dependency on experts, very recent research has started to explore tools that incorporate ideas from peer learning. Peer learning is a concept from cognitive psychology where students have the power to teach and learn from each other \cite{boud1999peer}. Prior work has uncovered that students who participate in peer learning perform better than students working on their own \cite{lundberg2003influence}, and were even better than students instructed by experts \cite{hinds2001bothered}. Very recent research has started to uncover that this learning method also appears to be suitable for crowd workers. Researchers have found that crowd workers enhance the quality of their work when they reviewed and provided feedback to the labor of other crowd workers  \cite{coetzee2015structuring, zhu2014reviewing, doroudi2016toward}. However, most of these approaches assume that requesters will be willing to take the time to redesign their tasks to incorporate and facilitate the peer learning model \cite{}. Under the current dynamics of Amazon Mechanical Turk, it is likely that requesters lack: a) the knowledge on how to effectively design tasks and workflows to help workers \cite{kulkarni2012turkomatic}; the time and incentives to want to improve tasks and worker satisfaction \cite{irani2013turkopticon}. Moreover, these studies made a trade-off between improving workers' labor quality and helping workers to reduce their  completion time \cite{kulkarni2012turkomatic}. Prior research focused on helping workers produce higher quality work but with the cost of increasing their completion times. For instance,  a very recent investigation explored workflows where novice workers provided feedback to each other by writing long writeups about each others' labor (800 to 1,000 characters long) \cite{doroudi2016toward}. While such workflows did help crowd workers to improve their performance, workers also had to invest 25\% more time in writing, reading and digesting each others' advice. But, most crowd workers are more interested in enhancing their skills to ultimately improve their salary than in increasing their work quality \cite{mason2010financial, martin2014being}. As explained above, increasing crowd workers' completion time per task can decrease workers' hourly wage. We believe that crowd workers might also be able to improve while on the job without sacrificing quality over completion time by providing quick, but selective peer advice. We consider this selective advice to be similar to coaching that is usually very direct and precise. 

Kittur et al. \cite{kittur2013future} envisioned that crowd markets could be a direct medium for skill development. \sys builds on this idea by helping workers to develop their skills without requiring experts to invest their time or requesters to redesign the tasks. Instead, \sys uses peer micro-advice to guide crowd workers to improve their performance, especially in working time without sacrificing quality. \sys also provides a quality assessment loop that dynamically finds high-quality peer advice (selective advice). 

%I can take a closer look at background later. For now, just pinning some sources that may be useful, depending on framing. 
%^also cite: sarasua2013microtask (about HITs based on CV)
%^may also be useful, but perhaps more related to other project: sarasua2014crowd (about "captures crowd workers’ interests, qualifications and work history, as well as requesters’ information")
%Also a number of sources about framing learning through work cited in \cite{billett2001learning} that might be useful
%Might want to frame in terms of motivation literature (to argue for why it's important to allow crowd workers to improve skills through their work)-- can \cite{kaufmann2011more} here, worker's motivation in crowdsourcing model. Can focus on idea of delayed payoffs and human capital advancement. Through this model, can also frame in terms of human capital advancement (so may want to cite other work related to human capital)
%also to consider: rogstadius2011assessment (crowdworker motivation improved when framed as helping others)

\subsection{Tools for Improving Crowdsourcing Platforms.}

Due to the inequalities between requesters and workers in AMT, workers usually obtain unfair treatment \cite{irani2013turkopticon, irani2016stories}. Researchers and practitioners have been exploring different browser extensions to improve the working conditions of crowd workers and reduce the inequalities. The web plugin of Turkopticon allows crowd workers to evaluate requesters after finishing their tasks \cite{irani2013turkopticon}. Turkopticon has become a useful tool for reducing the information asymmetry gap between workers and requesters (on AMT only requesters could officially rate workers). Other tools have explored enabling workers to help each other find higher hourly paying jobs to offset the fact that most crowdsourcing platforms do not provide an estimate working time of each task \cite{callison2014crowd}. TurkBench proposed a market visualization tool to help crowd workers to better 
manage their tasks \cite{hanrahan2015turkbench}. These novel tools have improved the working environment of crowd workers. In a similar fashion \sys aims to improve crowd workers' labor conditions by facilitating on-the-job skill development.  

\section{Designing \sys}
To design \sys we investigate: (1) the types of tasks that crowd workers want to improve in while working and workers' attitudes regarding knowledge-sharing on AMT; and (2) the types of peer micro-advice that workers provide for such tasks. We use the results of these two investigations to instruct the design of \sys and enable  on-the-job training on AMT. 

\subsection{Study 1: In What Tasks Do Crowd Workers Want to Improve?}
\subsubsection{Method.} To identify the types of tasks in which crowd workers want to improve we conducted a survey study. Our survey explored crowd workers' attitudes and impressions towards different types of tasks (HITs), how they tackled difficult HITs, types of HITs for which they wanted to become faster, HITs they wanted to complete with higher quality, and workers' motivations for becoming better at those particular HITs. We are also interested in workers' attitude about sharing knowledge with other workers.  %We also asked workers about their experiences in using online extensions or forums to tackle difficult tasks on AMT. 
The survey consisted of open-ended, multiple choice and Likert scale questions. To start to understand the types of HITs workers struggled with, we categorized existing HITs on AMT into 8 types based on the task typology from prior work \cite{ross2009turkers}, and provided examples of each task for clear illustration. 
% and asked participants detailed questions for each type.

%Participants average spent 18 minutes to finish the questionnaire. They were paid \$0.6 for the participation. 
We recruited 100 crowd workers from Amazon Mechanical Turk (AMT) to participate in our study. Our survey was open to all AMT workers and lasted around 15 minutes. We paid workers \$2 USD in line with current ethical standards on Mechanical Turk \cite{wearedynamo_2017}. We had a varied set of workers in our study: 40\% had finished over 10,000 HITs; 32\% had done more than 1,000 but less than 10,000 HITs; 28\% had finished less than 1,000 HITs. %36\% of participants had more than two years working experience on AMT, and 30\% had less than 6 months working experience on AMT. 34\% of participants worked more than 30 hours per week. 
%Workers in our study had over 500 HITs completed and over a 95\% acceptance rate. 


\begin{table}%
\caption{Simulation Configuration}
\label{tab:better}
\begin{minipage}{\columnwidth}
\begin{center}
\textbf{What types of tasks would you want to be better at? (i.e., tasks that you would like to do fast and with good quality.) You can choose more than one option. }
\begin{tabular}{ll}
  \toprule
  
  Audio transcription (e.g. transcribe up to 35 seconds of media to text)  & 49\\
  Writing (e.g. articles, summaries, reviews)       & 29\\
  Survey     & 25\\
  Image transcription (e.g. extract information from receipt)  & 18\\
  Data Collection (e.g. contact information on a website)    & 18\\
  Image tagging / labeling (e.g. facial attributes annotation)     & 15\\
  Categorization (e.g. select similar lipstick texture)  & 15\\
  Others & 2\\ 
  None     & 7\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering

\end{minipage}
\end{table}%

\subsubsection{Results.} 
Table \ref{tab:better} presents the type of tasks for which workers wanted to improve. Overall, workers seemed to want to improve in audio transcription tasks (n=49), followed closely by writing tasks (n=29). However, in the open-ended responses, workers expressed that although they saw room to grow their skills in writing tasks, they preferred to improve in audio transcription; especially because audio transcription tasks usually paid more than other tasks. As one worker explained: \emph{ ``There is good money in this [audio transcription tasks], especially if you do the longer tasks and can perform at a high level.''} Our participants also noted that: \emph{``Audio transcription can pay well, but one needs the necessary experience to perform the work quickly and efficiently.''}

%Figure \ref{fig:learnfrom} showcases that workers felt that when doing difficult tasks on AMT they not only learned new skills (e.g. learned how to better use excel, transcribe audio with better quality, or even develop programming skills), but they also developed new strategies on how to tackle difficult tasks and to use the mechanism of AMT properly. Moreover, from Fig \ref{fig:learnfrom} we observe that workers felt that solving difficult tasks also helped them understand themselves better and increases their self-confidence. This result suggests an opportunity for workers to improve if we can assist them to solve difficult tasks. 
%Read: plugin 43, forum 23
%Share forum 23, browser 20
%Updated: forum+facebook 
%Reading forum+facebook = 40
%share: forum+facebook = 42


Our survey also highlighted that a large proportion of workers used web plugins (72\% of the workers in our study) and online forums (57\%) to share or read advice about how to enhance their work experiences on AMT and grow professionally. For instance, workers frequently used Turkopticon \cite{irani2013turkopticon} to find ``friendly'' requesters. Participants noted that they usually obtained information about how to improve task performance from short forum postings, and they used browser plugins to learn about requesters or view customized AMT pages that better matched their needs and improved their work experiences (e.g., ``view the remaining HIT time in the pending task page''). The information from these web plugins was usually presented in short text snippets.  %Participants also noted that web forums usually required significant time investments to find relevant advice and because web plugins were not tailored for skill development they had to spend significant time configuring them to facilitate their professional growth. As one participant mentions: \emph{XX}.

\subsection{Study 2: What Types of Advice Do Crowd Workers Provide to Others?}
From our first survey, we saw that crowd workers already share and seek advice on related forums about how to complete tasks, thereby growing their skills and efficiency. However, this requires taking time away from their work on AMT. Moreover, from our pool we saw that novice workers usually had the hardest time finding peer advice especially because they did not even know what online sites to turn to or what other online workers to listen to (what advice to follow). 

We therefore started envisioning solutions where crowd workers could easily provide and access peer micro-advice while working. However, we did not know the type of advice that crowd workers would provide to each other while on the job. Would workers take this seriously and provide relevant advice to others? Or is the advice  irrelevant? Too specific? Too general? 

%In the design of \sys, our goal was to facilitate peer advice without having to spend time 
%aims are to allow workers read and provide advice while working. We believe that the advice especially benefits to novice workers, but potentially scalable to experienced workers. Although previous research has used a  ``real-time'' peer advice approach for crowd workers \cite{coetzee2015structuring},  we don't yet know the ``offline'' advice. For example, advice could be altogether irrelevant, too specific, or not specific enough. Moreover, we don't know how advice might vary according to the difficulty level of a given task. Filling in these knowledge gaps becomes especially important because we aim to introduce \sys as an inclusive tool designed with special attention to novice workers; where more experienced workers may breeze through certain tasks with no problems, novice workers may struggle and need additional help.

To better understand the nature of the advice that workers provide, we conducted a second study to analyze: (1) the type of advice that workers shared; and (2) the relationship between HIT difficulty and the advice content. In this second study, we focused exclusively on advice for audio transcription tasks given that a) they are one of the most common tasks on AMT \cite{hara2017data,difallah2015dynamics}, and b) our participants in Study 1 stated they most wanted to improve in audio transcription tasks.

\subsubsection{Method.} To inspect the types of advice crowd workers provide while on the job, we recruited crowd workers to a task that consisted of: (1) completing different audio transcription HITs; and (2) providing advice about how to do those tasks, especially with respect to improving speed and accuracy. Crowd workers provided advice via a free text form. 

To understand how advice might vary by level of task difficulty, and assess the feasibility of using \sys to provide on-the-job training using advice from workers of varying skill levels, we separated our crowd workers into three groups based on their self-reported levels of expertise with audio transcription: (1) novices; (2) some experience with audio transcription; (3) audio transcription experts. We assigned crowd workers audio transcription tasks that fit their self-reported levels of expertise, with the goal of gaining insights into whether crowd workers can provide relevant advice for tasks that match their knowledge levels. The tasks we assigned them are 25-second audio snippets of various difficulty levels. We assigned tasks as follows: (1) novices transcribed clear and slow audio snippets; (2) workers with some experience transcribed a normal speed lecture; (3) workers with substantial experience transcribed multi-speaker conversations; and (4) experts transcribed audio of speakers who are deaf, as this is a more challenging task \cite{bigham2017deaf}.  
% \cite{barefoot1993rating, hudgins1942investigation}).  
% We also asked  participants to provide feedback on how difficult they felt the audio transcription tasks were. 
We recruited a total of 80 participants from Amazon Mechanical Turk (20 for each type of audio transcription task). %This survey was distributed via Amazon Mechanical Turk to a group of 81 participants %(20 participants each audio resource, the only talk-show task had 21 participants). 
Workers took approximately 5 minutes in the study and were paid \$0.6 for their participation (in line with current ethical standards on Mechanical Turk \cite{wearedynamo_2017}). Workers produced 160 advice snippets (2 snippets per worker. One snippet of advice generally focused on how to become faster and the other on how to have more accuracy).

Next, we assessed the quality of the advice that workers. Here we were interested in understanding how the quality and nature of the advice might vary by level of difficulty and expertise. We were particularly interested in uncovering whether crowd workers could provide relevant advice while on the job. 

For this purpose, we hired three master workers from AMT (i.e., workers with over 500 HITs completed and over a 95\% acceptance rate) to independently classify the advice as either  relevant or irrelevant for becoming faster and/or more accurate in audio transcription tasks. First, two coders read through and classified each snippet of advice that workers produced as either ``on-topic'' or ``off-topic''. The two coders agreed on the classification of 153 pieces of advice (Cohen's \begin{math}\kappa = 0.832 \end{math}). We subsequently asked a third coder to act as a tiebreaker in cases of disagreement.


%After worke
%rs finished providing the advice we analyzed the quality of the advice. 
%\$3.6 USD in line with current ethical standards on Mechanical Turk \cite{}

%\begin{table}%
%\caption{Advice Categories}
%\label{tab:mapping}
%\begin{minipage}{\columnwidth}
%\begin{center}
%\begin{tabular}{ | p{4cm} | p{7cm} |}
 % \hline

  %Workflow advice    &Hard then return\\
   %                         &Listen once before write\\
    %                        &Listen one by one\\
    %                        &Pause \& play\\
    %                        &Re-listen after finish\\
    %                        &Read instructions\\
    %                        &Record on paper first\\
    %                        &Reread after finish (proofread)\\
    %                        &Skip and recheck\\
    %                        &Understand sentence rather than word by word\\
 % \hline
  %Software advice          &Using keyboard shortcut\\
   %                         &Slow down the audio using tools\\
  %\hline
  %Hardware advice          &Eliminate background noise\\
   %                         &Using headphone\\
    %                        &Using speaker\\
 % \hline
  %Psychological advice      &Focus on the tasks\\
   %                         &Keep open mind on audio resource\\
    %                        &Work slowly and careful\\
  %\hline
  %Long-term advice          &practice more on the same task\\
   %                         &Remember as more as possible\\
    %                        &Practice your typing speed\\

  %\bottomrule
%\end{tabular}
%\end{center}
%\bigskip\centering

%\end{minipage}
%\end{table}%

%\begin{figure}
%\centering
 % \includegraphics[width=1.0\columnwidth]{AdviceDistribution.png}
  %\caption{Overview of Crowd Bootcamp's design. }~\label{fig:advicedistribute}
%\end{figure}

\subsubsection{Results.} 
% We  found  that, independent of task difficulty and expertise of the advice-giver,  the  vast  majority (83\%) of the advice produced was relevant. Only 17\% of the advice was off-topic. 
% % off-topic advice was most common in the most simple audio transcription tasks. Workers might not have seen the value of providing advice for easy tasks, and hence left blank or irrelevant responses.
% Thus, across the board, and regardless of level of task difficulty or expertise, crowd workers were motivated to provide relevant advice. A sample of the relevant and off-topic advice provided for each type of task difficulty is presented in Table \ref{tab:result2}, as well as the median number of words used in the advice provided. Independent of task difficulty and expertise level, the advice provided oscillated between 13 and 14 words. 

% Overall, our second study shows that workers consistently provide relevant advice for audio transcription tasks regardless of task difficulty and their personal level of expertise. Next, we introduce \sys as a tool to help improve workers' working performance and skill development based on our findings.
% Next, we investigate \sys's impact on worker's working performance, especially when combining worker advice and growth mindset strategies. 

We  found  that, independent of task difficulty and expertise of the advice-giver,  the  vast  majority (83\%) of the advice produced was relevant. Only 17\% of the advice was off-topic.  A ratio of the relevant and off-topic advice provided for each type of task difficulty is presented in Table \ref{tab:result2}, as well as the median number of words used in the advice provided. Independent of task difficulty and expertise level, the advice provided oscillated between 13 and 14 words. 

Overall, our second study shows that workers can provide short and relevant advice for audio transcription tasks regardless of the task difficulty and their personal level of expertise. Next, we use these results to introduce \sys: a tool to facilitate peer micro-advice among crowd workers while on the job for professional development.%while improve workers' working performance and skill development based on our findings.


\begin{table}%
\caption{Advice Categories}
\label{tab:result2}
\begin{tabular}{ p{3cm} p{2.3cm} p{2cm} p{2.3cm} }
%\hline
%\multicolumn{3}{|c|}{Country List} \\
%\hline
{\bf \small Task Difficulty}& {\bf \small Percentage Relevant Advice} & {\bf \small Median Num. Words}& {\bf \small Example Relevant Advice}\\
\hline
\small Easy & \small 83\% & \small 13 & \tiny \emph{``Use headphones to try and listen to the audio better.''}\\
\small Medium Difficulty & \small 93\% &\small 14& \tiny  \emph{``If you want to get good at transcription HITS, do lots of them!''}\\
\small Medium Difficulty& \small85\% & \small 14& \tiny \emph{``1. Download the transcription audio. 2. Download and install Express Scribe. 3. Work on the transcription on Express Scribe.''}\\
\small Hard&\small 75\%&\small 14&\tiny \emph{``If you don't understand a word, don't get stuck there. Most likely you would understand it at the end when you know the context of the conversation.''}\\
\hline
\end{tabular}
\end{table}

\section{\sys}
We use the findings of our first two studies to design \sys. As a recap, our initial studies revealed that when crowd workers need extra help, they currently use time-intensive methods of searching in forums for peer advice. Participants also reported that they want to become better at audio transcription tasks. We also identified that crowd workers are able to provide relevant micro-advice while on the job.%, regardless of the task's difficulty.%skill level. 

% Previous studies showed that crowd workers produce better performance through real-time peer discussion \cite{zhu2014reviewing, coetzee2015structuring}. Also, other research proposed that crowd workers can improve their performance by reading an explanation of how other workers do on the same task with threshold \cite{doroudi2016toward}. They used the explanation length as a threshold, and only the explanations over 800 characters are qualified. Therefore, workers have to take longer time to complete the task because they have to wait for peer reply or read a long instruction.    

Armed with this knowledge, we present \sys, a web plugin (implemented as a Google Chrome extension) to help crowd workers' growth on Amazon Mechanical Turk by providing peer coaching. The coaching removes the need for workers to spend extra time outside AMT to develop themselves \cite{doroudi2016toward}, or for requesters to redesign their HITs to adapt to different skill levels \cite{gaikwad2017prototype}. Although we designed \sys to operate on any type of task, given the results from our prior studies, we choose to study \sys's applicability especfially to audio transcription tasks.

% We based \sys on our design probes that crowd workers improve after solving difficult tasks (e.g. audio transcription tasks). 
For a given AMT task, \sys displays short but useful peer advice to help workers improve their performance. The system is powered by crowd workers. It removes the need for requesters to have to invest time in learning how to best design their tasks to train workers and improve their  performance. 

\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{workflow_v2.png}
  \caption{The overview of \sys. There are two stages: 1) Crowd workers coach other workers; 2) Crowd workers receive peer coaching, and can upvote or downvote the coaching snippet. Through this dual feedback mechanism, \sys can select better coaching snippets. Moreover, an advice receiver can also be an advice provider}~\label{fig:workflow}
\end{figure}

To enable this, \sys has 3 main components: 1) Peer Coaching Collector, 2) Peer Coaching Selector (to select the coaching that is most useful), and 3) Coaching Display (to present workers with the most useful coaching). Figure \ref{fig:workflow} presents an overview of \sys.

\subsection{Peer Coaching Collector}
The Peer Coaching Collector module enables workers to input advice about how to improve at particular HITs (i.e., coach others). \sys's interface guides workers to provide advice especially about how to become faster and maintain good work quality. The collector lives as a plugin on AMT where workers can provide short snippets of advice about how one can improve at such type of work while doing a task. Unlike previous research \cite{doroudi2016toward} that leads workers to provide lengthy information, \sys focuses on guiding workers' to input micro-advice. We view this micro-advice similar to what a coach would briefly yell to players during a training or ``bootcamp'' to help them improve. 

For users of the plugin (Google Chrome extension), \sys shows a small ``give advice'' button on the bottom-left screen. Upon clicking the button, workers see a small window where they can provide their advice. Given the ``on-the-job'' nature of our intervention, we wanted to limit the cognitive load that we imposed on occupied workers. We thus limit the length of the advice to 100 characters. In the pop-up window, workers also select the type of tasks for which their micro-advice is relevant. Notice that although AMT tasks do provide description and titles, and we could have potentially used topic modeling or NLP techniques to categorize the tasks, prior work has indicated that such written information is not always the most relevant to classify tasks \cite{hara2017data}. We therefore focused our efforts towards a crowdsourced solution. Based on prior work \cite{hara2017data, ross2009turkers}, \sys considers that 8 main types of tasks exist on AMT: Audio transcription, Categorization, Data Collection, Image transcription, Image tagging / labeling, Surveys, Writing-related and Other. \sys's Peer Coaching Collector asks crowd workers to classify the tasks immediately after completing them into one of the eight specific HIT types. Through this process, we link micro-advice (coaching) to specific types of tasks. 



\subsection{Peer Coaching Selector }

For each type of task on AMT, \sys has a long queue of peer advice ready to coach crowd workers and help them improve. However, it is not clear whether all peer advice will actually prove beneficial. Especially with such a vast amount of advice data, relevant ``advice gems'' might get lost in the muck. To ameliorate this issue, \sys also has crowd workers provide micro-assessments of \sys's peer advice. 

\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{Interface.png}
  \caption{The \sys plugin for AMT workers to give, read and evaluate peer coaching. The dialog window on the bottom right side shows only after clicking the ``+'' green button. Crowd workers can share their advice to peers through the dialog box. \sys always displays peer coaching in a pop-up window on the top-right side when a worker accepts a HIT. Workers can use the left and right buttons to review different task-specific advice. Also, workers can provide their feedback through the ``upvote'' and ``downvote'' button in the peer coaching window. }
  \label{fig:interface}
\end{figure}

% 1. The FeedMe plug-in for Google Reader suggests friends, family, and colleagues who might be interested in seeing the post that
% you are reading. This user has selected john@doe.com and mary@email.com out of the list of 5 recommendations. The “Now” button
% sends an e-mail immediately; the “Later” button queues the item in a digest of multiple messages.

Our system adopts blind reviewing to evaluate the quality of the peer advice. \sys presents random advice to workers and has workers ``upvote'' or ``downvote'' the advice (see Figure \ref{fig:interface}). Although this advice is randomly selected in that it hasn't been curated or evaluated, note that it is advice that was previously linked to the type of task that the worker is currently doing.  When a piece of advice gets any feedback, it will win or lose ``credits'' (depending on whether it was upvoted or downvoted). These credits are pro-rated based on the reputation (explained momentarily) of the person providing the feedback. We considered that it was important to take into account the experience of the person providing the feedback, as they might have better insights about the utility of particular advice snippets on AMT. For this purpose, our web plugin also collects information about the number of tasks workers have done from AMT. 

The system calculates the reputation of feedback providers based on a) their experiences on AMT (number of tasks completed) and b) how similar their feedback is to the feedback provided by other workers. If a person's feedback deviates too much from  what others have inputted, we consider that such individual is giving  ``non-mainstream'' advice. Using this metric, we classify the advice given on \sys as either ``mainstream'' or ``non-mainstream,'' and rank mainstream advice based on peer ratings. In \sys, workers can customize whether they receive  mainstream or non-mainstream advice, and can view advice from workers with different experience levels. Through this mechanism, we enable workers to view common advice (mainstream) or advice with more unique perspectives (non-mainstream), as well as advice from people with varying experience levels (whose advice can be mainstream or non-mainstream). By default, \sys presents highly ranked mainstream advice first to workers. 
% Figure \ref{fig:interface} presents an overview of how workers see this advice. 
Through its voting mechanism, \sys can thereby present workers with advice that a vast majority of other workers found useful.  

\subsection{Coaching Display}
The Peer-Coaching Selector returns a list of advice snippets ranked according to workers' perspective of how useful the advice was. For a given task, the Coaching Display presents to workers the associated advice that was ranked highest in the list. \sys's Coaching Display for a given task showcases one of the most highly ranked advice snippets (mainstream advice, but people can also choose to view non-mainstream). If workers want more advice snippets, they can click the left or right button to review other peer-coaching. To ensure that new advice has the opportunity to be evaluated, \sys displays alongside the selected advice snippet a new piece of advice from the advice pool that needs feedback, and asks workers to evaluate the advice. Notice that workers can also choose to add their own advice for a given task. \sys keeps track of the advice that has already been shared with workers to avoid redudancy. Figure  \ref{fig:interface} presents how the coaching is displayed to workers. 

\section{Field Deployment and Evaluation}
%Our hypothesis is that \sys can lead crowd workers to grow professionally by helping workers to become faster at their labor and helping workers to produce higher quality labor. 
This paper hypothesizes that receiving selected peer coaching can lead to workers' growth while at work, measured in terms of an increase in workers' speed and labor quality. We therefore focus our evaluation on these claims: 

\begin{itemize}
  % We should compare whether our method better than the other methods. Especially compare to the crowd guided by the experts. 
  \item \sys enables workers to reduce their time to complete HITs, as compared to HITs of the same type
  \item \sys enables workers to improve the quality of their work, as compared to HITs of the same type
\end{itemize}

%[0604 Chun] Fro the results, the growth mondset group does not have any different than the original group, maybe we can illustrate it as a "how other researchers did than our contribution"
To study this hypothesis, we performed a field experiment on \sys users using five conditions: 1) a training where workers do tasks without receiving any type of peer coaching [control condition]; 2) a training where workers do tasks while receiving random peer coaching [random peer coaching condition]; 3) a training where workers do tasks while receiving selected peer coaching [\sys condition]; 4) a training where workers do tasks while receiving random peer coaching and exposure to growth mindset quotes [growth mindset condition]; 5) a training where workers do tasks while receiving selected peer coaching plus growth mindset quotes [\sys II condition]. 

Training conditions (4) and (5) focus on exposing workers to growth mindset ideas. We were inspired by research that identified that adding growth mindset quotes in video games facilitated students' growth \cite{o2014brain, o2016brain}. We were interested in exploring whether \sys coaching could be enhanced by integrating such mechanisms as well. Growth mindset quotes are short statements meant to inspire resilience and train people to think in terms of effort and strategies rather than innate talents or abilities \cite{o2011developing}; they tend to be generic, and all motivate one to persist in an action. In our field experiment, we used quotes such as, \emph{``Great works are performed, not by strength, but by perseverance''}, and \emph{``It does not matter how slowly you go so long as you do not stop''}.

%Notice that training conditions (4) and (5) focus on exposing workers to growth mindset ideas. We were inspired by research that identified that adding growth mindset quotes in video games facilitated students' growth \cite{o2014brain, o2016brain}. We were interested in exploring whether \sys coaching could be enhanced by integrating such mechanisms as well.  

%[0604 Chun] We should add other type of tasks in this paper to showcases our methods is not only for audio transcription. 
Our field experiment focused especially on training novice workers to improve in completing audio transcription tasks. A recent survey reported that audio transcription is the most popular task on Amazon Mechanical Turk \cite{difallah2015dynamics}, and workers in our study 1 also expressed this was an area in which they most wanted to improve. Honing audio transcription skills can substantially increase workers' wages; workers typically earn \$0.01-0.02 USD per sentence they transcribe \cite{novotney2010cheap}, which could potentially translate to high wages if a worker is fast (and accurate) enough. Specializing in audio transcription could allow crowd workers to command higher wages, as audio transcription is in high demand; written records of court proceedings and captions for live television events, such as the news, sports, and political speeches all require real-time audio transcription. Audio transcription skills are thereby highly specialized, highly valued, and well paid, earning up to \$300 per hour outside AMT. Building audio transcription skills on AMT can thereby help workers grow professionally and increase their earnings both in- and potentially outside of AMT.

\subsection{Field Experiment: Method}
To test out whether \sys provides better training method, we observed the real workers performance on AMT. For this field experiment, we aimed to help novice crowd workers, who were both new to AMT and inexperienced in audio transcription tasks. The field experiment had three audio transcription tasks. To better trace the user performance from task to task, participants interacted with our AMT-like website. The website recorded the working time and the accuracy of each task, and worker retention rate. To measure time to complete the task, we measured the time when a worker first accessed the task as the start time, and the time when workers submitted their labor (transcription) as their finish time. To study accuracy, we calculated the word error rate (WER) produced by each worker for each transcription, a commonly used metric to assess an audio transcription's performance. Moreover, to better understand users perspectives on \sys, participants who received peer coaching were asked to provide their feedback about the peer coaching with open-ended questions,

We have separated the participants into five training group. In the formal test, all participants were asked to complete an audio transcription task. After they finished one task, they can choose to start to do the next task or leave. They can do three tasks at most. Task audio resources were sourced from real world audio transcription HITs on AMT. The three audio sources were roughly commensurate difficulty, length, and level of instructions. Each audio were around 28 seconds. All three also involved equal levels of background noise, and the average speaking rate was 165 word-per-second.  

For each task, ``random peer coaching'' group received a random piece of advice that another worker generated. ``Selected peer coaching'' group received a piece of advice from other workers. However, the piece of advice was selected by our algorithms. We displayed different selected advice for different tasks. For the field experiment, we collected the peer advice before the training. Yet, in \sys, the selected peer coaching is dynamic in that it is dependent on the pool of workers who are assessing the peer advice. The best selected peer coaching varies based on users' feedback. In an experimental setting, the dynamic nature could confounding results. We used the advice we gathered in the study 2 as the peer coaching pool. Then, we recruited 30 workers on AMT to evaluated the peer coaching through up-voting and down-voting as the rules in \sys. We randomly assigned each worker 5 coaching snippets to evaluate.  Once workers had completed all the evaluations, we averaged the rating scores per snippet.

\subsubsection{Field Experiment: Participants}

The field experiment was conducted on AMT. We recruit the ``novice''  workers who had only completed less than 100 HITs. To reduce initial ability different between workers, we used a pre-test (which consisted of completing a real world audio transcription task) to included workers who finished tasks in a similar time and whose task accuracy is similar. 

After the pre-test, we recruited 150 participants on AMT, and randomly divided 30 participants into a group for the five experimental conditions. Participants in each condition were assigned the the same audio transcription tasks with the same order. Workers were paid \$0.6 for an audio transcription tasks (\$1.8 in total). 


% \subsubsection{Running the Field Experiment}
% %then explain how we distributed the advice to workers trying to complete the tasks
% We then conducted the field experiment to assess the efficacy of our tool in helping novice workers to complete audio transcription in a timely and accurate fashion. For the field experiment, participants in each condition interacted with a website we created that resembled AMT, thereby allowing us to better track their engagement with the tasks. 

% Using AMT, we recruited 150 total participants, divided into 30 novice workers (i.e., completing less than 100 HITs on AMT) for each of the five experimental conditions presented previously (control; random peer coaching; \sys; random peer coaching and growth mindset; \sys and growth mindset). We asked participants in each condition to complete the same three audio transcription tasks, and randomized participants between the 5 different conditions. In cases where workers were exposed to peer coaching we also asked them to complete a short survey after each task that questioned them about their perspectives on the peer coaching they had received. This survey helped us to better understand people's impressions of \sys. 

% To ensure that our workers were novice audio transcribers, we used a pre-test (which consisted of completing a real world audio transcription task), and only included workers with similar, novice-level completion times and accuracy levels. Workers were paid \$0.6 for completing each audio transcription tasks (\$1.8 in total). Workers could drop out whenever they wanted and their pay was pro-rated. 

% For each task, workers exposed to the random peer coaching received a random piece of advice that another worker had generated. %All workers with access to such coaching received for a given task the random advice. 
% Similarly, workers exposed to selected peer coaching received a piece of advice that another worker had generated and that peers had favored through our mechanism. All workers with access to selected peer coaching received the same selected advice for a given task. We compared worker performance by condition, using the time it took workers' to complete each task and the accuracy of their work (quality) as metrics. %Each audio transcription task consisted of listening to an audio segment and then writing out the content of the audio. 


% %Each of these tasks was of the same difficulty, consisted of transcribing 30 second audio clips. The tests consisted of completing real world audio transcription HITs collected from AMT. 
% To study the growth of crowd workers under each condition we measured: time to complete each task, and accuracy of the transcription (quality). To measure time to complete the labor (task), we measured the time when a worker first accessed the task as the start time, and the time when workers submitted their labor (transcription) as their finish time. To study accuracy, we calculated the word error rate (WER) produced by each worker for each transcription, a commonly used metric to assess an audio transcription's performance. 

% % To measure strategy use, we asked workers in each condition to mention any tactics or plans they had utilized to complete each audio transcription task, and qualitatively analyzed how people described the strategies they used.
% %about how much they were improving in audio transcription tasks. 
% %We ran the field experiment on AMT and recruited 90 novice crowd workers who had finished less than 100 HITs. To ensure that each group has workers with the same skill level for the audio transcribe task, we requested workers do a pre-test and ask for our main study only workers who completed the task in the same time and similar accuracy. Workers are paid \$0.6 for finishing each audio transcription tasks.


\subsection{Result}
During the study period, novice workers completed a total of 422 tasks across all 5 conditions. Some novice workers decided not to complete all the tasks and dropped out. However, the retention rates per condition were similar. At least 83 \% of the workers completed all the tasks in each condition. 

\begin{table*}[]
\centering
\caption{Comparison across conditions and worker performance in accuracy and completion time. The condition with the best performance for each question is in bold. Workers who receive \sys training outperformed other conditions in both accuracy and completion time. }
\begin{minipage}{\columnwidth}
\begin{center}
\label{tab:performancedetail}
\begin{tabular}{| p{2.8cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} |p{1cm} | p{1cm}| p{1cm}| p{1cm}|}
\hline
                & \multicolumn{4}{c|}{Accuracy}             & \multicolumn{4}{c|}{Completion time (sec)} \\
\cline{2-9}
                & Task 1 & Task 2 & Task 3 & Average & Task 1 & Task 2 & Task 3 & Average\\
\hline
Control         & 88.12\%    &   90.50\%  &   91.24\%   & 89.95\%  &    285   &    268     &    266 & 273                  \\
Simple advice   & 91.94\%    &   93.32\%  &   92.42\%   & 92.56\%  &    318   &    235     &    207 & 254                  \\
Growth mindset  & 90.46\%    &   91.95\%  &   \textbf{93.68}\%   & 92.03\%  &    301   &    274     &    198 & 258          \\
\sys & 92.62\%&\textbf{94.53\%}  & 92.80\%& \textbf{93.32\%}  &\textbf{227}&\textbf{182}&\textbf{151} & \textbf{186}             \\
\sys II & \textbf{93.43\%}& 93.55\%& 92.25\%&  93.07\%  & 282 & 201 & 164 &216             \\

\hline
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table*}

\subsubsection{Performance Analysis}
We were interested in workers' performance on audio transcription tasks. We studied performance based on workers' completion time and transcription accuracy. Table \ref{tab:performancedetail} presents the task accuracy and completion time for each task for different conditions.

From Table \ref{tab:performancedetail}, we observed that across conditions, the workers exposed to peer coaching had better accuracy than workers without peer coaching. We conducted a two way ANOVA to examine the effect of training method and accuracy (i.e., we examined whether the differences in accuracy across the 5 conditions in our study are statistically significant). We found that the differences in transcription accuracy across conditions was significant (F = 7.89, p = .00043). We also identified that there was no significant evidence that a particular audio transcription task affected people's accuracy within the condition (F = 1.85, p = .16 ). In other words, the accuracy differences appear to be related to whether workers received peer coaching, rather than to task content. Using Tukey test as post hoc analysis, we found that both the selected coaching condition (p < .0003) and random coaching condition (p < .012) significantly increased workers' accuracy when compared to workers who were not exposed to peer coaching. 

In summary, this first examination allows us to start to uncover that workers exposed to peer coaching had better accuracy than workers without access to such coaching. 

%the control group.    

From Table \ref{tab:performancedetail} we observe that workers exposed to selected peer-coaching were the fastest across all conditions. We conducted another two way ANOVA to inspect the effect of the peer coaching and task completion time (i.e., whether the differences in time completions across conditions were statistically significant). We also analyzed whether within conditions a task significantly affected task completion times. We found that for both task content (p < .0001) and training method (F = 7.043, p < .001 ) there was a statistically significant difference in completion time. In other words, receiving peer coaching (selected peer coaching, random peer coaching, etc.) reduced the time it took people to complete their work. Similarly, the task that people conducted also played a role in how much time they took. A post hoc Tukey test showed that workers exposed to selected peer advice took significantly less time to transcribe audio than people without access to any type of peer coaching (p < .004) and people exposed to random peer advice (p < 0.007). 

In summary, this second examination lets us identify that workers exposed to selected peer coaching were faster than workers without such coaching.

A two way ANOVA showed that workers receiving peer coaching had significantly better performance (accuracy and completion time) than workers without peer coaching (p < .001). As for the impact of integrating growth mindset quotes into workers' trainings, we did not find that there was a significant difference in workers' completion time or accuracy when exposed to growth mindset quotes (p = .32). %For accuracy, we find that the labor accuracy from \sys training workers are significantly better than the workers in control group (p <0.001). The growth mindset training not affect the accuracy of workers a lot (p = .32). That is, the peer coaching method influences more than growth mindset training method.   

Overall, workers with access to peer coaching were significantly more accurate in their jobs than workers without such coaching. Selected peer coaching appeared to be especially helpful for enabling workers to be faster at their job. Workers exposed to peer coaching were the fastest. Finally, we observed that our exploratory integration of the growth mindset training did not appear to have any affect in the short-term improvement of workers; we will reflect more on this result in the discussion.
%Overall, reading peer advice would improve novice workers audio transcription performance, especially in accuracy. Meanwhile, it would not trade worker's efficiency off for the accuracy. Novice workers who review the peer advice which voted by the workers would make them more accurate in audio transcription tasks and also reduce their working time than other training method.    

% \subsubsection{Retention Analysis}

% \begin{table*}[]
% \centering
% \caption{My caption}
% \begin{minipage}{\columnwidth}
% \begin{center}
% \label{tab:workernumber}
% \begin{tabular}{| p{3cm} |p{1.5cm}|  p{1.5cm}|  p{1.5cm}|}
% \hline
% \multicolumn{4}{|c|}{Number of worker}\\
% \hline
%                 & Start HIT & Finish \newline $\geq 1$ HIT & Finish\newline all HIT\\
% \hline
% Control         & 30 & 26 & 26\\
% Simple advice   & 30 & 29 & 27\\
% Selected advice & 30 & 27 & 25\\
% \hline
% \end{tabular}
% \end{center}
% \bigskip\centering
% \end{minipage}
% \end{table*}

% Table \ref{tab:workernumber} reports how many workers did at least one tasks, and complete all the tasks.   

% \subsubsection{Mindset Analysis}

%\subsubsection{Advice receiver feedback}
\subsubsection{Understanding Workers' Peer Coaching}

\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{feedback.png}
  \caption{A statistic of awarded usefulness in peer coaching based on the feedback from novice workers. 70\% of the of crowd workers think the peer coaching benefit them }~\label{fig:feedback}
\end{figure}
To better understand how workers perceived peer coach and why peer coaching, especially selected peer coaching, appeared to be helping workers to improve, we asked crowd workers who had received peer coaching to answer a short survey about their experiences. After completing a particular task and receiving the peer coaching, workers provided feedback about the coaching. The survey focused on probing workers about their impression on: 1) how the coaching helped them to improve their speed; 2) how the coaching helped them to improve their accuracy; 3) how the coaching affected them, in general. Workers' responded via a 5-point Likert scale and could also provided open-ended responses (but the free text response was optional). We received 173 feedback responses from workers in the random peer coaching condition and workers in the selected peer coaching condition. Figure \ref{fig:feedback} presents an overview of workers' perceptions of the peer coaching. Overall, 70\% of the feedback we received highlighted that they considered the peer coaching to be beneficial. Workers in the selected peer coaching condition pointed out that the coaching helped them to adopt better strategies: \emph{``I also re-tried the advice from the previous advice that was given of stopping the audio every 4-5 words, and since the speaker was really enunciating her words in this speech, that advice was also really helpful.''} %Upon closer inspection on the 

%70\% of feedback pictured that the peer advice was beneficial overall as Figure \ref{fig:feedback}. Some workers pointed out the advice really affect their strategy to the audio transcription tasks (e.g. \emph{I also re-tried the advice from the previous advice that was given of stopping the audio every 4-5 words, and since the speaker was really enunciating her words in this speech, that advice was also really helpful.} )



\section{Discussion and Future Work}

%In our survey, participants mentioned that audio transcription tasks pay well, but workers can earn from the tasks only if they have enough skills to do it quickly with acceptable quality. Yet most workers may lack mechanisms for improving and obtaining better opportunities \cite{deng2013crowdsourcing}. 
Our field study suggested that we can use peer micro-advice to help novice crowd workers to improve their skills while on the job, specifically with respect to improving accuracy and speed for audio transcription tasks. It appears that \sys can help workers to do more HITs per hour while simultaneously improving the quality of their work;  we conjecture that in turn, this could potentially reduce their chances of being rejected for producing low quality work. Together, this suggests that our system could especially help novice crowd workers to improve their hourly pay on AMT while developing their skills.  

It is expected that in the future, crowd markets will become employment hubs where increasingly large numbers of workers with varying expertise and levels of skills compete for employment and contribute to projects. It therefore becomes important to envision mechanisms that help the workers of these platforms to continuously grow and obtain better opportunities \cite{deng2013crowdsourcing}. Our first survey highlighted how workers currently have to invest time outside AMT to read up on strategies to improve and grow.  With many crowd workers needing to use all of their time just to make ends meet \cite{paolacci2010running, berg2015income, durward2016crowd, thies2011paid}, it is clear that not all workers can easily take time off their labor to improve themselves. Our field study suggested that we can use peer coaching to help workers improve speed and accuracy at their job without needing to leave their job or take time off, a mechanism that can be especially beneficial for workers from marginalized communities who cannot afford to invest time off work. With \sys, we show that for a specific type of highly valued task on crowd work--- audio transcription tasks--- even short snippets of ``micro-advice'' that don't overwhelmingly distract from the task at hand can improve workers' skills and performance. Moreover, with \sys, workers of all levels of experience can successfully contribute to helping other workers to improve their skills. The mechanisms behind \sys are themselves crowdsourced, conferring benefits to both crowd workers (who can improve their skills while on the job) and requesters (who needn't manually re-design tasks to guide workers of varying skill levels). 

In the future, we would also like to explore systems that leverage coaching from successful workers for even more specialized tasks. We can envision that if most future labor occurs online, we could then request micro-coaching from more complex professions such as CTOs or Managers. We could then use an approach similar to \sys to obtain such micro-advice to help novices become better at the online job of their choice. 

Prior research has identified that the order of micro-tasks impacts performance \cite{cai2016chain}; that having spaced repetitions usually impacts how many words a person can learn on their own for vocabulary acquisition \cite{edge2011micromandarin}; and that mixing tasks with varied difficulty and similarity type impacts learning \cite{koedinger2012knowledge}. In the future, we plan to explore inter-mixing peer coaching with the automatic generation of ``lists of tasks to do.''  Helping workers to select the tasks that might be most beneficial for them while pairing them with the best peer-advice might enable workers to grow even more. 

However, in the short term, we believe that \sys could be adapted to other domains. What type of tasks should a worker be doing to become one of the highest paid workers on AMT? Can we get experienced crowd workers (e.g., super turkers \cite{hara2017data}) to provide coaching to novices to make a better living with AMT?  On this same note, platforms could potentially recommend coaching from specialized workers to become more skilled in specific areas while still earning money within AMT. 

We extended the microtasking platform to generate coaching that could enable crowd workers to improve while getting paid. However, exactly \textit{how} these types of paid trainings fit within the work dynamics and practices of crowdworkers remains an open question. It is possible that workers might not want to follow the advice of our system. For instance, they might prefer doing tasks in their own way because it is more entertaining. %The greater long-term benefits of developing a new skill may be enough to motivate workers to follow \sys's training. 
In addition, the way in which we present the benefits of \sys to workers may influence workers' performance. Helping workers to visualize the expected long-term benefits of improving at their job may enable workers to take more-informed decisions on whether they should invest the time and effort in reading and following the peer coaching. Future work could explore interfaces that learn through time how to present peer coaching to workers to motivate them to follow the coaching.

\sys provides selected peer micro-advice to novice workers for improvement. However, being exposed to peer coaching could also limit or shutdown workers' thought process and ideas on how to do a specific task. It is possible this could lead workers to believe that their approach is not best, as it is different than what others recommend, thereby discouraging workers from using creative approaches to solve tasks.  In the future we are also interested in exploring how to enable coaching that helps workers to improve, but also promotes workers' initiative and creativity. %Therefore, we could also study whether the \sys can guide crowd worker improve in the tasks which require creative workers, such as logo design.

% What helped workers' be faster and produce higher quality labor the most was the peer-coaching, especially the \sys's selected peer coaching

%on surface information and predicted learning costs and benefits. 

%who want to be like them.

% Assume the growth mindset help
% Another of our main insights is that the selected peer advice contains the element for improving growth mindset. Moreover, crowd workers who read random peer advice and train their growth mindset simultaneously can perform as well as the crowd workers who read selected peer advice. This is very helpful for the design of our system. For the advice which does not have adequate review to determine whether the advice is useful or not, we can provide with growth mindset training to achieve a similar effect of selected advice.   

In the design of \sys, we were interested in enabling mechanisms through which workers could grow. Inspired by prior work \cite{o2014brain} that identified that incorporating growth mindset incentives helped learners to better solve difficult tasks, we also explored combining \sys with growth mindset  trainings. However, our field deployment illustrated that adding growth mindset quotes into workers' trainings did not have a significant effect on workers' improvement. Still, we believe growth mindset could have potential to positively impact skill building and task performance on AMT and other crowd work platforms. It could be, for example, that exposure to growth mindset training could have a long term, but not short term impacts on workers' motivations and behaviors on crowd work platforms. Future work could further explore the application of growth mindset training to crowd workers' experiences using more longitudinal study designs.
 

\subsection{Limitations}

The insights from this paper are limited by the methodology used and the population that was studied. While we used real tasks from crowd marketplaces, and also recruited real novice crowd workers, our results might not yet generalize and apply to crowd work at large. Moreover, our pretest to guarantee that all the participants have similar skills means that we only tested our system with novices, and can only evaluate the benefits accordingly; we cannot speak to whether \sys could be suitable for more experienced workers, even though our ultimate goal is to provide a tool that can scale to different levels of experience. \sys may also have possible novelty effects that need to be studied in greater depth in future work by conducting longitudinal studies. 

\section{Conclusion}
This paper introduced \sys, a Chrome extension to promote skill building and professional development by assisting novice crowd workers to increase their speed and accuracy in completing audio transcription tasks on AMT. Informed by two studies we undertook to understand how and where crowd workers want to grow their skills, and how they approach the idea of giving feedback on a specific type of task to other crowd workers while on the job, \sys uses peer micro-advice and a twofold reputation mechanism to help workers improve their skills. \sys differentiates itself from prior work in improving skills for crowd workers by depending on the crowd workers themselves (regardless of AMT experience or skill level) rather than requesters or external experts to generate the help. Moreover, \sys innovates on related work by embedding the help mechanisms within tasks so that work growth can be achieved while on the job, and by providing meaningful, useful advice through micro-tips rather than lengthy and comprehensive assistance. In this way, our system grounds itself in the practical concerns and constraints that both crowd workers and requesters face, such as limited time and resources available to devote to improving skills or task workflow designs. Although our exploration of growth mindset training did not show significant results, with \sys, we show an alternative and promising approach allowing crowd workers to improve their skills and ultimately, grow professionally in their careers. The present study sets the stage for future work in designing crowd work that supports rewarding careers that allow workers to grow and advance in their skills and careers over time through their work on crowd work platforms.


% Bibliography
\bibliographystyle{ACM-Reference-Format}
\bibliography{sample-bibliography}

